A Unified Approach to Sparse Signal Processing

A unified view of sparse signal processing is presented in tutorial form by bringing together various fields. For each of these fields, various algorithms and techniques, which have been developed to leverage sparsity, are described succinctly. The common benefits of significant reduction in sampling rate and processing manipulations are revealed. The key applications of sparse signal processing are sampling, coding, spectral estimation, array processing, component analysis, and multipath channel estimation. In terms of reconstruction algorithms, linkages are made with random sampling, compressed sensing and rate of innovation. The redundancy introduced by channel coding in finite/real Galois fields is then related to sampling with similar reconstruction algorithms. The methods of Prony, Pisarenko, and MUSIC are next discussed for sparse frequency domain representations. Specifically, the relations of the approach of Prony to an annihilating filter and Error Locator Polynomials in coding are emphasized; the Pisarenko and MUSIC methods are further improvements of the Prony method. Such spectral estimation methods is then related to multi-source location and DOA estimation in array processing. The notions of sparse array beamforming and sparse sensor networks are also introduced. Sparsity in unobservable source signals is also shown to facilitate source separation in SCA; the algorithms developed in this area are also widely used in compressed sensing. Finally, the multipath channel estimation problem is shown to have a sparse formulation; algorithms similar to sampling and coding are used to estimate OFDM channels.

==> Arash.txt <==
Acronym: 		CT : Computer Tomography
		 	PPM: 	Pulse Position Modulation
			FM: 	Frequency Modulation

Uppercase to lowercase in the Table

2*#Desired    in the table
Refence #44 need attention
Zayed2001 as same as the above line
Marvasti1992
Feichtingerbook1994
Grochenig must be well written
Grochenig2001 ..>> Chapter in the Dr. book
Appendix A is written in the word file43.
Marvastibook_chapRandom2001 !!
Change Unser's paper please.
Marvastibook_chapErrorCorection2001 should be changed as the above chapters


Figs. 30 & 31 should be ghanged RDE >>>>> IDE


I (Vahid) must put 2 citation from Remi.(ValiolahZade sent them me)

VERY IMPORTANT: IN THE ACRONYMS RDE HAS BEEN CHANGED TO IDE, BUT ITS PLACE IN THAT TABLE IS WRONG!
